Supervised Time Series Classification for Anomaly Detection in Subsea Engineering

Time series classification is of significant importance in monitoring structural systems. In this work, we investigate the use of supervised machine learning classification algorithms on simulated data based on a physical system with two states: Intact and Broken. We provide a comprehensive discussion of the preprocessing of temporal data, using measures of statistical dispersion and dimension reduction techniques. We present an intuitive baseline method and discuss its efficiency. We conclude with a comparison of the various methods based on different performance metrics, showing the advantage of using machine learning techniques as a tool in decision making.

==> Images/5_DT_images/DT_algorithm_bis.tex <==
\tikzset{bigbox/.style={draw, rectangle, rounded corners, thick, node distance=7em, text width=25em, text centered, minimum height=13em}}
\tikzset{box/.style={draw, rectangle, rounded corners, thick, node distance=7em, text width=9em, text centered, minimum height=4em}}
\tikzset{smallbox/.style={draw, rectangle, rounded corners, thick, node distance=7em, text width=9em, text centered, minimum height=3em}}
\tikzset{every picture/.style={/utils/exec={\sffamily}}}
\begin{document}

\forestset{
  L1/.style={sibling distance=19mm, fill=Cerulean}
}

\begin{forest}
    for tree={
        draw = MidnightBlue,
        grow=0,reversed, % tree direction
        parent anchor=east,child anchor=west, % edge anchors
        edge={line cap=round},outer sep=+1pt, % edge/node connection
        rounded corners,minimum width=25mm,minimum height=8mm, % node shape
        l sep=10mm, % level distance    
        s sep=30mm}
  [Data set,L1[Training data,L1][Test data,L1]]
  \draw[-Stealth] (4.9, 2) -- (5.35, 2);
  \draw[-Stealth] (5.6, 2.9) -- (6.1, 2.9);
  \draw[-Stealth] (4.9, -1.9) -- (8.15, -1.9);
  \draw[-Stealth] (9.95, -0.35) -- (9.95, -1.1);  
  \draw[-Stealth] (9.7,2.9) -- (10.2,2.9);
  \draw[-Stealth] (8.15,0.7) -| (7.9, 2.1);
  \draw[-Stealth] (12,2.1) |- (11.75, 0.7);
  \node [bigbox, color = OliveGreen] at (9.95, 2) {};
  \node [box,  color = OliveGreen, fill = SpringGreen] at (7.9, 2.9) {\textcolor{black}{Measure purity and select the best feature using ASM}};
  \node [box, color = OliveGreen, fill = SpringGreen] at (12, 2.9) {\textcolor{black}{Split the data set into smaller subsets}};
  \node [box, color = OliveGreen, fill = SpringGreen] at (9.95, 0.7) {\textcolor{black}{Repeat recursively for each child node}};
  \node [box, color = RedOrange, , fill = YellowOrange] at (9.95,-1.9) {\textcolor{black}{Test the model on unseen data}};
  \node [color=black] at (9.95, 4) {Generating the decision tree};
\end{forest}

\end{document}

==> Images/5_DT_images/horizontal_DT_bis.tex <==
\begin{document}
\tikzset{box/.style={draw, rectangle, rounded corners, thick, node distance=7em, text width=19em, text centered, minimum height=6.5em}}
\tikzset{container/.style={draw, rectangle, dashed, inner sep=2em}}
\tikzset{line/.style={draw, thick, -latex'}}
\forestset{
  L1/.style={fill=Cerulean,},
  L2/.style={fill=OrangeRed,edge={darkgray,line width=0.5pt}},
  L3/.style={fill=Green,edge={darkgray,line width=0.5pt}},
  L4/.style={fill=pink,edge={darkgray,line width=0.5pt}},
}
\begin{forest}
    for tree={
        grow=0,reversed, % tree direction
        parent anchor=east,child anchor=west, % edge anchors
        edge={line cap=round},outer sep=+1pt, % edge/node connection
        rounded corners,minimum width=25mm,minimum height=8mm, % node shape
        l sep=10mm % level distance
    }
  [Root node,L1
    [Decision node,L2
        [Leaf node,L3][Leaf node,L3]
    ]
    [Decision node,L2
        [Decision node,L2
            [Leaf node,L3][Leaf node,L3]
            ][Leaf node,L3]
    ]]
    \path [line] (1.35, -1.5) -- (1.35, -0.1);
    \node [color=black] at (1.4, -1.8) {Splitting};
    \node [color=black] at (2, 1.3) {1};
    \node [color=black] at (5.4, 1.9) {2};
    \node [color=black] at (5.4, 0.6) {3};
    \node [color=black] at (5.2, 2.6) {Branch/sub-tree};
    \node [box, color = darkgray] at (5.2, 1.2) {};
\end{forest}
\end{document}

